An Empirical Evaluation of the Implementation of the California Consumer Privacy Act (CCPA)

On January 1, 2020, California passed the California Consumer Privacy Act (CCPA) by more than 56% of voters intended to enhance privacy rights and consumer protection for residents of California, United States. Since then, more conditions have been added to the Act to support consumers' privacy. In addition, two years after the first effective day of CCPA, consumers have seen California organizations apply approaches to adapt to CCPA. Many organizations quickly upgrade their policy to comply with the legislation and create effective platforms such as data portals that allow consumers to exercise their privacy rights. However, on the other hand, we still noticed aspects of CCPA being absent on some websites. Additionally, we found no prior evaluation of the CCPA implementation in organizations. Therefore, the convergence of the regulatory landscape and the organization's privacy policy needs to be studied. This paper was about an empirical evaluation of the implementation of the California Consumer Privacy Act. The report includes the evaluations of the following industries: social media, financial institutions, mortgages, healthcare providers, and academic institutions. Our approach was to set up a criteria table constructed from the CCPA Act and then use that table as a checklist while reviewing a company's privacy notice. Finally, we concluded this paper with an online tool application design that verifies the CCPA implementation. Upon completion, the application would be free to use so consumers can quickly inspect a website for CCPA compliance. Additionally, it is an advising tool that a website admin can utilize to enhance CCPA compliance for their website. The conjunction of this empirical report and a practical application function as a stimulus to promote CCPA implementation in organizations and deliver awareness to consumers about privacy rights they can demand.

==> Implementation.tex <==

\section{Project Implementation - CCPA Verifier 1.0 }
\label{sec:implemetation}
\subsection{Backend application}

The backend server is written in Java and follows using a microservices pattern. The application is constructed by four major java packages: Main application file, controller package, manager package, model package, and service package. The below figure describes how we structure our application.

\begin{figure} [h]
    \centering
    \includegraphics{images/application_structure.png}
    \caption{Caption}
    \label{fig:my_label}
\end{figure}

The main application file is the start-up file that the application uses to execute the first functions. The service package contains standalone and reusable functionality that the app uses to check CCPA criteria on the website. For example, the generic CCPA service class has functions to look for notice of collection, CCPA link, right to access, right to delete, and opt-out. For more complicated websites which require a hybrid data crawling solution (manual direct the application which pages to crawl data first), we can extend the generic CCPA service to create a website-specific version of CCPA service. For example, we can create a CCPA service named ChaseCPPAService that specifically contains crawling functions working with the Chase website. To write an extended function is simple; we only need to input a URL that points to the site's CCPA privacy page directly to skip the automatic CCPA searching process that the generic CCPA function does. That approach would ensure the application can always reach the CCPA privacy page when facing a complex website structure. After that, the remaining natural language processing process can still be automated by the generic CCPA module. 
We usually do not need to override the CCPA criteria look-up functions in most cases. Currently, our application service package contains the following classes:  GenericCCPAService class, GoogleCCPAService, FacebookCCPAService, and ChaseService. We will add more classes to the application as the application needs to check more websites. We believe this project would benefit our community in the long term, so we aim to maximize the reusability and make the application more maintainable. 

Next, the manager package combines standalone services to satisfy application business requirements. For example, when consumers perform CCPA checking on a website, the application needs to execute a set of tasks that include looking for a privacy notice first, then CCPA notice, then right to access, right to delete, and right to opt-out. Therefore, we use the manager class to schedule these functions' execution and then generate a complete result that includes data fields to indicate if the privacy notice page exists, the CCPA page exists, and CCPA rights exist. The result is packed in a model class called CCPAResult. After the result is generated, the manager classes return it to the controller getting the data ready to transfer to a front-end application. 

The last package in our application is the controller package. It is the gateway that the backend application receives web requests from a front-end application. The data is served under JSON format. To request data, the front-end application will send a REST request to the endpoint with the website URL as the request parameter. For performance, all the CCPA criteria checking would be performed using a single REST request, so we only have two API endpoints now. One is used for the CCPA checking, and the other one is used to retrieve browser screenshots for the front end. 

\subsection{Front End Application}
The front-end application allows consumers to interact with the backend app using a graphical user interface. The front-end app is deployed on a cloud webserver. The website is developed as a single web page application with material design to give consumers an intuitive experience. The website is hosted at this URL: www.ccpaverifier.com. The homepage will present brief CCPA information to advertise the privacy law. The website structure consists of a landing page, a feature page for CCPA checking, a team information page, and a contact page.

\subsubsection{Landing Page}
The landing page is the first location consumers will experience when visiting the website. The landing page also includes other nested pages because of the nature of a single-page application (SPA). Therefore, the beauty of that is to allow consumers to scroll down to discover more website content without being redirected to other pages. In addition, SPA will enable consumers to take less time to understand the website structure. Only the feature page on which consumers perform CCPA checking on other websites is located on another page. 

\begin{figure}[H]
    \centering
    \includegraphics[width=1\textwidth]{images/landingPage.png}
    \caption{Landing page}
    \label{fig:my_label}
\end{figure}

\subsubsection{How It Works Page}

This section introduces the features that our application offers. The first feature redirects consumers to the full CCPA document. The second feature allows consumers to select a website from a given list and then perform the CCPA verification. The last feature will enable consumers to enter the URL of any website. The backend server will execute a generic CCPA verifying function to try its best to retrieve a result. If the application can generate the result, it will render the result on the website. Otherwise, the front-end application would present an error to notify consumers that the verifying process is failed and ask them to try another URL. 

\begin{figure}[H]
    \centering
    \includegraphics[width=1\textwidth]{images/howitworks.png}
    \caption{How it works page}
    \label{fig:my_label}
\end{figure}

\subsubsection{CCPA Information Page}
This section presents essential information about CCPA, such as subjects that CCPA applies to, consumers' rights, and penalties that organizations may receive if they do not implement CCPA. This module aims to provide consumers who visit the site a quick preview of CCPA. If consumers want to know more about CCPA, they can follow the link on our site to read a full CCPA document.
\begin{figure}[H]
    \centering
    \includegraphics[width=1\textwidth]{images/ccpainfopage.png}
    \caption{CCPA infomation page}
    \label{fig:my_label}
\end{figure}

\subsubsection{Contact Us}
Our application is still in developmental phase so we would like to receive feed backs to improve design as well as functionalities. Therefore, we include an contact form on our website and let consumers submit questions,feed-backs or report error. Based on the response, we will tweak and improve our application overtime.
\begin{figure}[H]
    \centering
    \includegraphics[width=1\textwidth]{images/contactuspage.png}
    \caption{Contact us page}
    \label{fig:my_label}
\end{figure}



==> accessbility.tex <==
\section{Accessibility Support}
We also enhanced our website to make it compatible with assistive technology for disabled people. We have to make necessary changes to the colors and layout of our application UI. To know which web application components we should revise, we evaluated accessibility support using Screen Reader - Assistive Technology: NVDA \cite{NVDA}, WAVE Web Accessibility Evaluator Tool \cite{WAVE}, Color Contrast Analyzer \cite{Color-Contrast-Analyzer"}. The result that these programs generated provided us with suggestions for improving our website interface. 

\begin{itemize}
    \item \textbf{Visual focus}: Used by sighted keyboard-only users to identify their location on the page. The tool found on our website has a low visual focus which means users will have difficulty seeing which element has focus. For example, when we hover the mouse on the feature button, read more button, back to top button, the focus is not visible enough for people who have vision-impairing to see. 
    \item \textbf{Keyboard Operable}: When collapsing the browser's window into a smaller window, the navigation menu collapses into a hamburger button. Consumers cannot use either keyboard and mouse to navigate the web page.
    \item \\textbf{Announcement}
        \begin{itemize}
            \item Linkedin buttons are announced as lists when they are buttons, and the link destination is not announced
            \item Text lists are not formatted as lists. Assistive technology users will have difficulty identifying the text is related
            \begin{figure}[H]
                \centering
                \includegraphics{images/text_list_accessbility.png}
                \caption{Text list is not compatible with assistive technology}
                \label{fig:my_label}
            \end{figure}
        \end{itemize}
        
    \item \textbf{Link}: Links open in new window without advanced warning. Assistive technology users will have difficulty navigating back to the website (can be fixed with title attribute for the link in the code)
    \begin{figure}[H]
        \centering
        \includegraphics{images/card_accessbility.png}
        \caption{A link issue }
        \label{fig:my_label}
    \end{figure}
    \item \textbf{Headings }: Assistive technology users often navigate the page with headings
        \begin{itemize}
            \item Headings don’t have a logical order.
                \begin{figure}[H]
                    \centering
                    \includegraphics{images/heading_accessbility.png}
                    \caption{Headings do not have a logical order}
                    \label{fig:my_label}
                \end{figure}
            \item Heading levels are skipped
                \begin{figure}[H]
                    \centering
                    \includegraphics{images/heading_accessbility_2.png}
                    \caption{Heading levels are skipped}
                    \label{fig:my_label}
                \end{figure}
        \end{itemize}
    \item \textbf{Alt text }:  used to describe images to assistive technology users
        \begin{itemize}
            \item First image on home page contains text. Assistive technology users cannot determine the purpose of the image (if the image is decorative, can set alt to decorative (alt=””)) Note: If the image relays the same information as a text paragraph on the website, We should mark it as decorative since it’s a visual representation of the information. 
            \begin{figure}[H]
                \centering
                \includegraphics{images/Alt_text.png}
                \caption{Alt text issue}
                \label{fig:my_label}
            \end{figure}
        \end{itemize}
\end{itemize}

Based on the accessibility report, we began to adjust our website layout and design to be better compatible with assistive technology. Upon completing the adjustment, people with disabilities can use assistive technology to use our website. We believe it is crucial to let disabled people access our application to be aware of the rights that CCPA provides. Regardless of people's conditions, consumers get affected in the same way in term of data collection and sharing made by organizations 

==> business_requirement.tex <==
\section{ Application Business Requirement}
\label{sec:business_requirement}
\subsection{Scope}
\begin{enumerate}
    \item Project Scope
    \begin{itemize}
        \item Initial system
        \begin{itemize}
            \item Will be a single page application web application
        \end{itemize}
        \item Initial Browser Support
        \begin{itemize}
            \item Will support latest version of Chrome, Firefox or Edge
        \end{itemize}
        \item Initial Data
        \begin{itemize}
            \item Website URL : The application will accept website URL as input string to perform CCPA verifying function  
        \end{itemize}
        \item Permission for collecting user data 
        \begin{itemize}
            \item To monitor the application performance, the application may record the following data from consumers :
            \begin{itemize}
                \item IP address
                \item Fail and Successful operations
                \item Website URL being checked
                \item Responding time
            \end{itemize}
        \end{itemize}
    \item In Scope Functionality
    \begin{itemize}
        \item Presenting of CCPA Information
        \item CCPA Compliance Verifier 
        \item Instruction To Exercise CCPA Rights
        \item Instruction To File CCPA Compliant 
    \end{itemize}
    \item Out of Scope Functionality
        \begin{itemize}
            \item Develop an Android version of the application
            \item Allow consumers to perform mass checking on multiple websites at same time. 
        \end{itemize}
    \end{itemize}
    
    \item Constraints
    \begin{itemize}
        \item Time
        \begin{itemize}
            \item Our final deadline is May 15
            
        \end{itemize}
        \item Resources
        \begin{itemize}
            \item Our team is compiled of one member
        \end{itemize}
    \end{itemize}
\end{enumerate}

\subsection{Project Function and Non-functional Requirements}


\begin{center}
\setlength{\mycolwidth}{\dimexpr \textwidth/2 - 2\tabcolsep}%
\begin{longtable}{|p\mycolwidth|p\mycolwidth|}
\caption{Function and Non-functional Requirements } \label{ccpa:long}\\
\hline 
\multicolumn{1}{|c|}{\textbf{Functional Requirements}} & \multicolumn{1}{c|}{\textbf{Non Functional Requirements }}\\ \hline 
\endfirsthead

\multicolumn{3}{c}%
{{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\
\hline 
\multicolumn{1}{|c|}{\textbf{Functional Requirements}} & \multicolumn{1}{c|}{\textbf{Non Functional Requirements }}\\ \hline 
\endhead

\hline \multicolumn{3}{|r|}{{Continued on next page}} \\ \hline
\endfoot
\hline \hline
\endlastfoot
    \hline
    One web page is used to house the application
    
    & \\
    \hline
    The page changes to display a new section based on user interactions.
    
    & Page loading of a new section of the web app should take less than 3-second \\
    \hline
    The web application is deployed on a cloud server to allow anyone to access the page online.
    
    & Cloud service should not take down our application for daily maintenance any longer than thirty minutes\\
    
    \hline
    Cloud service should be resistant to most common attacks.
    
    & \\
    

    
    \hline
    The application should have a modular design to allow any part to be modified without needlessly affecting any other part.
    
    & \\
    
    \hline
    The part should be built in a way to allow a unit test to be created for each. 
    
    & \\
\end{longtable}
\end{center}

\subsection{Business Requirements (Core Components)}
\subsubsection{Security}
\begin{itemize}
    \item \textbf{Background}: Current version of the application does not save any user data because we are not offering user creating or logging in. Therefore, there is no risk of leaking data. However, the application still utilizes HTTPS protocol to encrypt the data transferred between the back-end server and the front-end application. 
    In addition, the back-end application should only receive requests from our domain at ccpaverifier.com and reject requests from other domains to protect data integrity and the back-end server itself. Cross-Origin Resource Sharing (CORS) technique will be used for that purpose.
    \item \textbf{Actor}: Consumers.
    \item \textbf{Precondition}: The program is released, and consumers start to input the website URL into a typing box.
    \item \textbf{Post condition}: The website URL is encrypted using SSL and sent over port 443. Results, including screenshots, would be transferred back to the source using the same method.
    \item \textbf{User Stories:} "As a consumer, I want the data that I send and receive to and from the back-end server to be encrypted  and must not be seen or modified by anyone"
    \item \textbf{Business Rules:}
    \begin{itemize}
        \item Encrypt transferred data.
        \item The application should be able to handle penetration testings using the OWASP framework or similar frameworks.
        \item Man in Middle cannot read the data transferred between source and destination. The result cannot be altered.
        
    \end{itemize}
    \item \textbf{Pass Criteria:}
    \begin{itemize}
        \item Transferred data can only be  encrypted and decrypted at the front-end app and back-end server.
        \item Website can survive from DDOS attack or other common web attacks.
    \end{itemize}
    
    \item \textbf{Fail Criteria:}
    \begin{itemize}
        \item Data is not encrypted before being transferred over the internet. Attacker can read the transferred data.
        \item The web server cannot resist common wed attacks. 
    \end{itemize}

\end{itemize}

\subsubsection{Presenting of CCPA Content}
\begin{itemize}
    \item \textbf{Background}: This feature includes two components. First, the website will display brief CCPA information. Second, if consumers want to learn more about CCPA, they can click on button which contains a link on the website to redirect themselves to the official page of CCPA  under  Office of Attorney General website. 
    \item \textbf{Actor}: Consumers.
    \item \textbf{Precondition}: The website is up and running. Consumer can access the homepage.
    \item \textbf{Postcondition}: Consumers can read information about CCPA or visit the official CCPA website
    \item \textbf{User Stories:} "As a consumer, I want to learn about CCPA to understand which organizations it applies to and my rights"
    \item \textbf{Business Rules:}
    \begin{itemize}
        \item Our website must display information about CCPA in a readable format
        \item Our website must redirect consumers to official CCPA  page immediately when consumers click on the button which contain a link.
        \item  
        \begin{center}
\setlength{\mycolwidth}{\dimexpr \textwidth/2 - 2\tabcolsep}%
\begin{longtable}{|p\mycolwidth|p\mycolwidth|}
\caption{Function and Non-functional Requirements } \label{ccpa:long}\\
\hline 
\multicolumn{1}{|c|}{\textbf{Functional Requirements}} & \multicolumn{1}{c|}{\textbf{Non Functional Requirements }}\\ \hline 
\endfirsthead

\multicolumn{3}{c}%
{{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\
\hline 
\multicolumn{1}{|c|}{\textbf{Functional Requirements}} & \multicolumn{1}{c|}{\textbf{Non Functional Requirements }}\\ \hline 
\endhead

\hline \multicolumn{3}{|r|}{{Continued on next page}} \\ \hline
\endfoot
\hline \hline
\endlastfoot
    \hline
   After visiting the home page, the user can scroll down to read essential information about CCPA. 
    
    & CCPA information is displayed in an easy-to-read font and appropriate font size \\
    \hline
    To access the official CCPA website to learn more about CCPA, consumers need to click on an arrow button in the content holder of "Information about CCPA."
    
    & The arrow button will appear as soon as consumers hover the mouse on the content holder component \\
    
   
\end{longtable}
\end{center}
    \end{itemize}
    \item \textbf{Pass Criteria:}
    \begin{itemize}
        \item Summarized information about CCPA is presented correctly and clearly
        \item Consumers are redirected to official CCPA  website  upon request
    \end{itemize}
    
    \item \textbf{Fail Criteria:}
    \begin{itemize}
        \item The website failed to display CCPA information.
        \item the website failed to redirect consumers to official CCPA site .
    \end{itemize}

\end{itemize}

\begin{figure}[H]
    \centering
    \includegraphics[width=40mm]{images/ccapinfoflow.png}
    \caption{Presenting of CCPA Information Flow}
    \label{fig:my_label}
\end{figure}
\subsubsection{CCPA Compliance Verifier}
\begin{itemize}
    \item \textbf{Background}: This feature allows consumers to choose a website from a list or enter their own URL to verify CCPA compliance of the website. Then the application will utilize  web crawling Selenium to check if it can find keywords that match the list of CCPA requirements. 
    \item \textbf{Actor}: Consumers.
    \item \textbf{Precondition}: The website available to access. Consumers can click on the accessing feature button to use the CCPA verifier. 
    \item \textbf{Postcondition}: CCPA verifier will provide consumers result after finishing CCPA verifying function. 
    \item \textbf{User Stories:} "As a consumer, I want to pick a website from the list to verify if that website complies with CCPA", " As a consumer, I want to enter a website URL to check if that website complies with CCPA" 
    \item \textbf{Business Rules:}
    \begin{itemize}
        \item The application must present a result to consumers in no longer than one minute.
        \item The application must show an error if back-end server is not working or consumers submit wrong URL.
        \item The application must generate correct result.
        \item The result the application presents to user must be freshly generated at the time of submission. It means the result must be original, not be stored prior to the current session then retrieved.  
        \item If the application decides that the tested website complies with CCPA, our application must present a link to the CCPA page. Then consumers will able to use that link to exercise their CCPA rights. 
        \begin{center}
\setlength{\mycolwidth}{\dimexpr \textwidth/2 - 2\tabcolsep}%
\begin{longtable}{|p\mycolwidth|p\mycolwidth|}
\caption{Function and Non-functional Requirements } \label{ccpa:long}\\
\hline 
\multicolumn{1}{|c|}{\textbf{Functional Requirements}} & \multicolumn{1}{c|}{\textbf{Non Functional Requirements }}\\ \hline 
\endfirsthead

\multicolumn{3}{c}%
{{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\
\hline 
\multicolumn{1}{|c|}{\textbf{Functional Requirements}} & \multicolumn{1}{c|}{\textbf{Non Functional Requirements }}\\ \hline 
\endhead

\hline \multicolumn{3}{|r|}{{Continued on next page}} \\ \hline
\endfoot
\hline \hline
\endlastfoot
    \hline
    Consumers can either choose a website from the list or enter a website URL manually. The front-end app will send a request to the back-end server to perform CCPA verifying tasks. 
    
    &  User can enter website URL with our without prefix 'http://www.' The application can detect the missing parts and add them automatically. \\
    
    \hline
    If CCPA is found on the tested website, the application shows a link for consumers to exercise  CCPA rights, such as how to request data access, data deletion, or opt-out of sale. 
    & The front end UI shows the "click here" button that redirects the user to the CCPApage of the tested website. \\
     
    \hline
    If CCPA is not found on the website being tested, the application lets consumers download a result of a screenshot and then shows instructions on how to file a complaint to the Office of the Attorney General.
    &
    The front-end interface shows the "Show Instruction" button that displays a dialog box instructing consumers how to file a complaint. 
    
    \hline
    The function is asynchronous, so consumers can still interact with other UI components during the ongoing verifying process. 
    
    & While waiting for a response, the application will display spinning wheels to let users know the process is still ongoing  \\
    
   
\end{longtable}
\end{center}
    \end{itemize}
    \item \textbf{Pass Criteria:}
    \begin{itemize}
        \item The application can present a result when finishing verifying CCPA on a website
        \item The application can present a screenshot of the tested website 
        \item The application can present a link for consumers to exercise CCPA rights if the website complies with CCPA
        \item The application can show instructions for filing a complaint if the tested website does not comply with CCPA.
        
    \end{itemize}
    
    \item \textbf{Fail Criteria:}
    \begin{itemize}
        \item The application displays an error because the back-end server does not respond
        \item It takes longer than the expected amount of time for the back-end server to respond to the request
        \item The web application gives incorrect results compared with a result acquired manually.
    \end{itemize}

\end{itemize}

\begin{figure}[H]
    \centering
    \includegraphics{images/ccpa_verifying_flow.png}
    \caption{CCPA Criteria Verifying Flow}
    \label{fig:my_label}
\end{figure}




==> design_doc.tex <==

\section{Design}
\label{sec:design}
\subsection{Dependency Diagram}
This section presents a dependency diagram of our web application. The dependency diagram explains how different application features rely on each other. For example, feature A depends on feature B. When feature B is unavailable, feature A will not work as specified in the business rule. According to the dependency diagram, a notice of collection checking, right to know to check, right to delete checking, and right to opt-out of sale matching feature rely on the CCPA notice checking feature, which relies on privacy notice checking. Then the features which offer assistance to exercise CCPA rights, filing CCPA complaints, and capturing a screenshot of the result all depend on the CCPA rights checking mentioned earlier.
\begin{figure}[H]
    \centering
    \includegraphics[width=1\textwidth]{images/dependency_diagram.png}
    \caption{Dependency Diagram of Features}
    \label{fig:my_label}
\end{figure}


\subsection{High Level Flow Diagram}
\subsubsection{Introduction}
This section explains the flow of the data with high-level architecture. We have divided our web application into different layers, and each of them handles the data flow in our application. Our application consists of six layers: UI, Router, Data Handler, and Service. Each of these layers takes a request and return a variety of response depending on the given request. A layer communicates directly with its surrounded layers only to lower the complexity level of our web application. We will explain the behavior of each layer in detail later. In addition to those layers, some layers affect multiple layers directly. There is security and error handling. The technology that the back-end uses to communicate with the front-end is REST \cite{restapi}
\begin{figure}[H]
    \centering
    \includegraphics[width=1\textwidth]{images/network_diagram.png}
    \caption{High-Level Architecture diagram}
    \label{fig:my_label}
\end{figure}


\subsubsection{User Interface Layer (UI)}
The front-end of our web application is what we use to present visual content to consumers. This layer directly interacts with the user and accesses the server to fulfill the valid request. It forms a request, sends it to the server, and renders any response received from the server.

\subsubsection{Service Layer}
The service layer consists of standalone services that meet the consumers' requests. It takes input from the manager layer and processes it before returning the result. It may use the lower level to store and access data if necessary. Standalone services should be as general as possible so we can reuse them in other parts of the application.


\subsubsection{Security}
Considering security in high-level design is critical to protect our servers and ensure the integrity of the result generated by the application. Although the application does not save sensitive data in this version, the impact generated by the application must be encrypted before transferring to avoid being altered. We enforce using HTTPS protocol between the front-end and back-end servers to do that. HTTPS protocol uses public-private key infrastructure to encrypt and decrypt information when sending and receiving data. \\
In addition, the cloud servers need to be secured to avoid being attacked. We only allow necessary ports opened, and the back-end server only accepts requests from our front-end domain using a cross-origin resources sharing (CORS) policy. To make the server even more secured, we think about allowing only US IP addresses to access our website. Then it may help put the website out of the radar of hackers outside the US.

\subsubsection{Error Handling Rules}
\begin{itemize}
    \item Business Logic : 
    \begin{itemize}
        \item When consumers attempt to connect to the server when it is offline, the application will show an error letting the consumers know the back-end server is not functioning. 
        \item When consumers submit an invalid website address, the application will return a not found or bad input error and then ask consumers to submit again. 
    \end{itemize}
    
    \item UI
    \begin{itemize}
        \item When consumers y to input invalid data, the application will raise an exception as a result of invalid behavior
    \end{itemize}
    
    \item UI and Business Logic 
    An exception will be raised when the users try to act on application-specific business rules. Custom exceptions appropriate to a situation will be raised to produce a descriptive error message to users and administrators
    \end{itemize}

\subsubsection{Network Architecture Diagram}
In this network architecture design, we provide a high-level network architecture diagram. It explains the overall process of data flow in our networking system. The chart consists of the following network components:
Client
DNS server
Front-end firewall
Front-end web server
Back-end firewall
Back-end web server
Generally, we deployed our back-end and front-end apps on two different virtual machines and let them communicate over the internet. Separating the two servers, it will make the system more extensible. In the future, we can develop an Android or iOS application that will talk to the same back-end app. In addition, when doing maintenance, we can work on either application without disturbing the other application. 
\begin{figure}[H]
    \centering
    \includegraphics[width=1\textwidth]{images/Network_Architecture_Diagram.png}
    \caption{Network Architecture Diagram}
    \label{fig:my_label}
\end{figure}

\subsection{Low Level Designs}
This section includes diagrams showing the data flow through the feature and its error handling charts. These diagrams are used to explain the features we are currently building and the mistakes in certain areas.
\subsubsection{CCPA Verifier}
This design will show the data flow of the CCPA Verifying feature. Two scenarios may happen when executing the CCPA verifier. In the first scenario, If a CCPA privacy notice is found on the tested website, the application will perform additional functions such as checking for the right to access, delete, and opt out. Then the application will return a link to the CCPA page of the website, where consumers can exercise their CCPA rights. In the second scenario, if the application cannot find any information related to CCPA on the tested website, it will allow consumers to download a screenshot of a website and then instruct consumers to file a complaint to the Office of Attorney General. 

\begin{figure}[H]
    \centering
    \includegraphics[width=1\textwidth]{images/CCPA Verifier Sequence Pass.png}
    \caption{CCPA Verifier Sequence Diagram -  CCPA Found }
    \label{fig:my_label}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\paperwidth]{images/CCPA Verifier Sequence Fail.png}
    \caption{CCPA Verifier Sequence Diagram - CCPA Not Found }
    \label{fig:my_label}
\end{figure}

==> fasle_positive_negative.tex <==
\section{False Positive and False Negative Issues}
Fundamentally, the business logic behind the CCPA verifier function utilizes web crawling and natural language processing. To determine if a website complies with CCPA, our application needs to detect a required number of keywords that match a set of  CCPA criteria. If a website does not implement  CCPA but mentions the right keywords, the verifier will make a false assumption. Therefore, our application logic would falsely determine that website complies with one or more CCPA criteria. On the other hand, our application will also face some false-negative cases.\\
Another issue comes from the sensitive keyword matching algorithm that our application is powered by. We have a bucket of keywords required to match each CCPA criteria. However, suppose a website uses keywords for  CCPA implementation which are different from our keywords. Again, our application would make false assumptions and then conclude the website does not comply with CCPA. In short, the false positive and negative issue depends on how we define boundaries for the keywords. 
The figure below is an example of a false positive case our application faced. We used our CCPA verifier to test our website, ccpaverifier.com, and it returned a wrong result. We do not have CCPA implementation on our website in this scenario, but the application logic still detected that our website complies with some CCPA criteria. However, because our website has many keywords about CCPA, it makes the CCPA verifier misunderstand that our website was implementing CCPA.

\begin{figure}[H]
    \centering
    \includegraphics[width=1\textwidth]{images/wrong_result.png}
    \caption{An example of CCPA false positive}
    \label{fig:my_label}
\end{figure}

Consequently, we believe in limiting these false positive and negative issues; we will keep improving our back-end logic to make the web crawler better navigate through websites. If the crawler can navigate correctly to the privacy pages rather than elsewhere, it will likely come up with the correct determination. In addition, understanding a website context is more valuable than checking exact keywords. If we can find an approach to make, our application recognizes that if a website mentions CCPA by extracting the content, we will get much more accurate results. To do that, an AI technique, natural language processing (NLP), is what we should look at for our future research. NLP will allow our application to analyze and understand the context of a document and then decide if that document is relevant to a topic based on a confidence score. Therefore, the general concept seems to be ideal for our application. It can be in our next developmental stage in the future. 

==> project_plan.tex <==
\section{Project Roadmap}
This section presents a road map of our project. Generally, we started developing the Java back-end application using Selenium and Springboot on January 25. Since then, we have added the features to verify CCPA notice, a notice of collection, the right to access data, delete data, and opt-out of sale. Then, on March 13, we started developing a front-end application using the VueJS framework. Then when we finished everything on April 3, we deployed both front end and back end apps on Namecheap cloud server for public access. Since then, we will continuously evaluate and add more supported websites to the CCPA Verifier application.
\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\paperwidth]{images/ProjectRoadMap (1).png}
    \caption{Project Road Map}
    \label{fig:my_label} 
\end{figure}


==> signature.tex <==
\vspace*{1in}
\begin{center}
\section*{SIGNATURE PAGE}
\addcontentsline{toc}{section}{Signature Page}

\end{center}
\vspace{0.50in}

\newcommand\blank[1]{\rule[-.2ex]{#1}{.4pt}}

\begin{flushleft}

\begin{tabular}[t]{ll}
\setlength{\tabcolsep}{12pt}

\vspace{0.25in}
\textbf{\uppercase{Project:}} & \hspace{7mm}\makecell[tl]{\uppercase{AN EMPIRICAL EVALUATION \\OF THE IMPLEMENTATION\\ OF THE CALIFORNIA CONSUMER PRIVACY ACT \\(CCPA) }} \\

\vspace{0.25in}
\textbf{\uppercase{Author:}} & \hspace{7mm}\makecell[tl]{Trong Nguyen} \\

\vspace{0.25in}
\textbf{\uppercase{Date Submitted:}} & \hspace{7mm}\makecell[tl]{Spring 2022\\Department of Computer Science} \\

\vspace{0.25in}
\makecell[bl]{Mohammad Husain, Ph.D.
\\Project Committee Chair\\Computer Science} & \hspace{7mm}\makecell[bl]{\blank{8cm}} \\

\vspace{0.25in}
\makecell[bl]{Tingting Chen, Ph.D.\\Computer Science} & \hspace{7mm}\makecell[bl]{\blank{8cm}} \\

\end{tabular}


\end{flushleft}

==> timetable.tex <==
\section{Tentative Timetable}
\label{sec:timetable}

\begin{center}
\begin{tabular}{|p{10cm}|c|}
\hline
Deliver Proposal & 01/18/2021 \\
\hline
CCPA Checking Application Design Completed & 4/15/2022 \\
\hline
CCPA Checking Application Implementation Completed & 5/22/2022 \\
\hline
CCPA Checking Application Testing Completed   & 5/30/2022 \\
\hline
CCPA Checking Application Deployment Completed  & 6/10/2022 \\
\hline
Project first draft sent to advisor & 6/30/2022 \\
\hline
Project first draft sent for committee review & 7/14/2022 \\
\hline
Project second draft completed & 8/8/2022 \\
\hline
Project Defense & 8/31/2022 \\
\hline
\end{tabular}
\end{center}

==> title.tex <==
\vspace*{1in}

\thispagestyle{empty}
\begin{center}

\textbf{\uppercase{AN EMPIRICAL EVALUATION OF THE IMPLEMENTATION OF THE CALIFORNIA CONSUMER PRIVACY ACT (CCPA) \\}}

\vspace{0.75in}
A Project\\Presented to the\\Faculty of\\California State Polytechnic University, Pomona

\vspace{0.75in}
In Partial Fulfillment\\Of the Requirements for the Degree\\Master of Science\\In\\Computer Science

\vspace{0.75in}
By\\Trong Nguyen\\2022

\end{center}

==> toc.tex <==
\section*{Tentative Thesis Table of Contents}
\label{sec:toc}

\begin{enumerate}
  \item Abstract
  \item List of Figures
  \item Acknowledgments
  \item Glossary
  \item Introduction
  \begin{enumerate}[A.]
    \item Motivation
    \item Problem Description
    \item Research Goals
    \item Web Crawler and existing CCPA tools 
    \begin{enumerate}[i.]
      \item Java Selenium
      \item Consumer Privacy Interactive Tool 
      \item Cookiebot
    \end{enumerate}
    \item Structure of Thesis
  \end{enumerate}
  \item Methodology
  \begin{enumerate}[A.]
    \item Description of CCPA Compliance Web App Tool Design . 
    \item Implementation of CCPA Tool description
    \item Description of CCPA Tool Deployment 
    \item CCPA Tool Test Description
    \item CCPA Tool Test Result 
  \end{enumerate}
  \item Evaluation of Results
  \item Conclusions and Future Work
  \item References
\end{enumerate}
